The rotate-plus-shift C-arm trajectory: Complete CT data with less than 180{\deg} rotation

In the last decade C-arm-based cone-beam CT became a widely used modality for intraoperative imaging. Typically a C-arm scan is performed using a circle-like trajectory around a region of interest. Therefor an angular range of at least 180{\deg} plus fan-angle must be covered to ensure a completely sampled data set. This fact defines some constraints on the geometry and technical specifications of a C-arm system, for example a larger C radius or a smaller C opening respectively. These technical modifications are usually not benificial in terms of handling and usability of the C-arm during classical 2D applications like fluoroscopy. The method proposed in this paper relaxes the constraint of 180{\deg} plus fan-angle rotation to acquire a complete data set. The proposed C-arm trajectory requires a motorization of the orbital axis of the C and of ideally two orthogonal axis in the C plane. The trajectory consists of three parts: A rotation of the C around a defined iso-center and two translational movements parallel to the detector plane at the begin and at the end of the rotation. Combining these three parts to one trajectory enables for the acquisition of a completely sampled dataset using only 180{\deg} minus fan-angle of rotation. To evaluate the method we show animal scans acquired with a mobile C-arm prototype. We expect that the transition of this method into clinical routine will lead to a much broader use of intraoperative 3D imaging in a wide field of clinical applications.

==> MyTeXMacros.tex <==
% Test
%%%%%%%

\newcommand{\dbar}{{\mkern3mu\mathchar'26\mkern-12mu d}}
\newcommand{\dbarVec}{{\mathchar'26\mkern-13.5mu\dVec}}
\newcommand{\gammabar}{{\mkern3mu\_\mkern-9mu\gamma}}


% Auxiliary
%%%%%%%%%%%%

\newcommand{\Note}[1]{xxxx #1 xxxx}
\newcommand{\mkpage}[2]{\mbox{}\marginpar{\raggedleft\hspace{0pt}--#1--\tiny #2}}
\newcommand{\mkmargin}[1]{\mbox{}\marginpar{\raggedleft\hspace{0pt}\small #1}}
\newcommand{\half}{\tfrac{1}{2}}
\newcommand{\Mathematica}{\textsf{\textsl{Mathematica\ }}}
\newcommand{\mkdelta}{{\scriptstyle \Delta}}
\newcommand{\Nabla}{\boldsymbol\nabla}
\newcommand{\Transpose}{{\text T}}
\newcommand{\eff}{{\text{eff}}}



% Vector notation
%%%%%%%%%%%%%%%%%%

\newcommand{\aVec}{{\boldsymbol a}} \newcommand{\AVec}{{\boldsymbol A}}
\newcommand{\bVec}{{\boldsymbol b}} \newcommand{\BVec}{{\boldsymbol B}}
\newcommand{\cVec}{{\boldsymbol c}} \newcommand{\CVec}{{\boldsymbol C}}
\newcommand{\dVec}{{\boldsymbol d}} \newcommand{\DVec}{{\boldsymbol D}}
\newcommand{\eVec}{{\boldsymbol e}} \newcommand{\EVec}{{\boldsymbol E}}
\newcommand{\fVec}{{\boldsymbol f}} \newcommand{\FVec}{{\boldsymbol F}}
\newcommand{\gVec}{{\boldsymbol g}} \newcommand{\GVec}{{\boldsymbol G}}
\newcommand{\hVec}{{\boldsymbol h}} \newcommand{\HVec}{{\boldsymbol H}}
\newcommand{\iVec}{{\boldsymbol i}} \newcommand{\IVec}{{\boldsymbol I}}
\newcommand{\jVec}{{\boldsymbol j}} \newcommand{\JVec}{{\boldsymbol J}}
\newcommand{\kVec}{{\boldsymbol k}} \newcommand{\KVec}{{\boldsymbol K}}
\newcommand{\lVec}{{\boldsymbol l}} \newcommand{\LVec}{{\boldsymbol L}}
\newcommand{\mVec}{{\boldsymbol m}} \newcommand{\MVec}{{\boldsymbol M}}
\newcommand{\nVec}{{\boldsymbol n}} \newcommand{\NVec}{{\boldsymbol N}}
\newcommand{\oVec}{{\boldsymbol o}} \newcommand{\OVec}{{\boldsymbol O}}
\newcommand{\pVec}{{\boldsymbol p}} \newcommand{\PVec}{{\boldsymbol P}}
\newcommand{\qVec}{{\boldsymbol q}} \newcommand{\QVec}{{\boldsymbol Q}}
\newcommand{\rVec}{{\boldsymbol r}} \newcommand{\RVec}{{\boldsymbol R}}
\newcommand{\sVec}{{\boldsymbol s}} \newcommand{\SVec}{{\boldsymbol S}}
\newcommand{\tVec}{{\boldsymbol t}} \newcommand{\TVec}{{\boldsymbol T}}
\newcommand{\uVec}{{\boldsymbol u}} \newcommand{\UVec}{{\boldsymbol U}}
\newcommand{\vVec}{{\boldsymbol v}} \newcommand{\VVec}{{\boldsymbol V}}
\newcommand{\wVec}{{\boldsymbol w}} \newcommand{\WVec}{{\boldsymbol W}}
\newcommand{\xVec}{{\boldsymbol x}} \newcommand{\XVec}{{\boldsymbol X}}
\newcommand{\yVec}{{\boldsymbol y}} \newcommand{\YVec}{{\boldsymbol Y}}
\newcommand{\zVec}{{\boldsymbol z}} \newcommand{\ZVec}{{\boldsymbol Z}}

\newcommand{\muVec}{{\boldsymbol\mu}} \newcommand{\MuVec}{{\boldsymbol\Mu}}
\newcommand{\lambdaVec}{{\boldsymbol\lambda}} \newcommand{\LambdaVec}{{\boldsymbol\Lambda}}
\newcommand{\omegaVec}{{\boldsymbol\omega}} \newcommand{\OmegaVec}{{\boldsymbol\Omega}}
\newcommand{\rhoVec}{{\boldsymbol\rho}} 
\newcommand{\nablaVec}{{\boldsymbol\nabla}}


\newcommand{\bbbVec}{{\boldsymbol\bbb}}
\newcommand{\etaVec}{{\boldsymbol\eta}}
\newcommand{\psiVec}{{\boldsymbol\psi}}
\newcommand{\tttVec}{{\boldsymbol\ttt}}                 
\newcommand{\TTTVec}{{\boldsymbol\TTT}}                  
\newcommand{\xxxVec}{{\boldsymbol\xxx}}   


% Statistical operators
%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\EEE}{{\mathrm E}}                           %  Expectation
\newcommand{\Var}{{\mathrm Var}}                         %  Variance
\newcommand{\Cov}{{\mathrm Cov}}                         %  Covariance
\newcommand{\Law}{\mathcal L}                           %  Law
\newcommand{\Binomial}{\mathcal B}                      %  Binomial
\newcommand{\Poisson}{\mathcal P}                       %  Poisson
\newcommand{\Normal}{\mathcal N}                        %  Normal



% Functions
%%%%%%%%%%%

\DeclareMathOperator{\erf}{erf}
\DeclareMathOperator{\lb}{lb}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\vec2}{vec}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\sinc}{sinc}
\DeclareMathOperator{\jinc}{jinc}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\rect}{II}
\DeclareMathOperator{\shah}{III}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator*{\argmax}{argmax}



% Transform operators
%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\Re}{{\rm Re}}
\renewcommand{\Im}{{\rm Im}}
\newcommand{\Radon}{{\mathsf R}}
\newcommand{\XRay}{{\mathsf X}}
\newcommand{\Fourier}{{\mathsf F}}
\newcommand{\FourierLeftArrow}{\stackrel{\displaystyle\Fourier}{\longleftarrow}}
\newcommand{\FourierRightArrow}{\stackrel{\displaystyle\Fourier}{\longrightarrow}}
\newcommand{\Hankel}{\mathsf H}
\newcommand{\AnnotatedLeftRightArrow}[1]{\stackrel{\displaystyle #1}{\longleftrightarrow}}
%\newcommand{ \HankelLeftRightArrow}{\AnnotatedLeftRightArrow\Hankel}
\newcommand{\FourierLeftRightArrow}{\AnnotatedLeftRightArrow\Fourier}
\newcommand{\Abel}{\mathsf A}
\newcommand{\Identity}{\mathsf 1}


% IQ stuff
%%%%%%%%%%

\newcommand{\SSP}{{\mathrm SSP}}                         %  SSP

\newcommand{\PSF}{{\mathrm PSF}}                         %  PSF
\newcommand{\PSFx}{\PSF\!_{\text x}}                    %  PSF_x
\newcommand{\PSFy}{\PSF\!_{\text y}}                    %  PSF_y
\newcommand{\PSFz}{\PSF\!_{\text z}}                    %  PSF_z
\newcommand{\PSFr}{\PSF\!_{\text r}}                    %  PSF_r

\newcommand{\LSF}{{\mathrm LSF}}                         %  LSF
\newcommand{\SSF}{{\mathrm SSF}}                         %  SSF
\newcommand{\ESF}{{\mathrm ESF}}                         %  ESF

\newcommand{\MTF}{{\mathrm MTF}}                         %  MTF
\newcommand{\MTFx}{\MTF\!_{\text x}}                    %  MTF_x
\newcommand{\MTFy}{\MTF\!_{\text y}}                    %  MTF_y
\newcommand{\MTFz}{\MTF\!_{\text z}}                    %  MTF_z
\newcommand{\MTFr}{\MTF\!_{\text r}}                    %  MTF_r

\newcommand{\NPS}{{\mathrm NPS}}                         %  NPS
\newcommand{\DQE}{{\mathrm DQE}}                         %  DQE
\newcommand{\SNR}{{\mathrm SNR}}                         %  SNR 
\newcommand{\CNR}{{\mathrm CNR}}                         %  CNR 
\newcommand{\SPR}{{\mathrm CNR}}                         %  SPR 


% CT specific
%%%%%%%%%%%%%
\newcommand{\RF}{R_{\text F}}                           % R_F
\newcommand{\RM}{R_{\text M}}                           % R_M
\newcommand{\RD}{R_{\text D}}                           % R_D
\newcommand{\RFD}{R_{\text{FD}}}                        % R_FD=R_F+R_D
\newcommand{\aaa}{\alpha}                               % Projection angle
\newcommand{\aaahhh}{\mkdelta\aaa_{\text H}}            % Angle equivalent of slice thickness
\newcommand{\aaasss}{\mkdelta\aaa_\sss}                 % Angle equivalent of slice thickness
\newcommand{\aaaR}{\aaa_{\text R}}                      % Reconstruction position alpha_R
\newcommand{\aaaw}{\bar\aaa}                            % Projection angle
\newcommand{\bbb}{\beta}                                % Angle in fan
\newcommand{\cccR}{c_{\text R}}                         % Reconstruction position c_R
\newcommand{\ddd}{d}                                    % Table increment
\newcommand{\Eeff}{E_\eff}                              % Effective energy 
\newcommand{\mueff}{\mu_\eff}                           % Effective mu
\newcommand{\fff}{{\mathit\Phi}}                        % Fan angle
\newcommand{\geff}{g_\eff}                              % Geometric efficiency
\newcommand{\kFan}{l}                                   % Fan-beam kernel
\newcommand{\kPar}{k}                                   % Parallel beam kernel
\newcommand{\ppp}{p}                                    % Projection data
\newcommand{\ppoly}{p_{\text{poly}}}                    % p_poly
\newcommand{\pmono}{p_{\text{mono}}}                    % p_mono
\newcommand{\Teff}{t_{\text{eff}}}                      % Effective scan time
\newcommand{\Trot}{t_{\text{rot}}}                      % Rotation time
\newcommand{\ttt}{\vartheta}                            % Projection angle
\newcommand{\tttR}{\ttt_{\text R}}                      % Reconstruction position theta_R
\newcommand{\TTT}{\Theta}                               % Projection angle in Fourier domain
\newcommand{\seff}{S_{\text{eff}}}                      % Effective slice thickness
\newcommand{\sss}{S}                                    % Slice thickness
\newcommand{\xxx}{\xi}                                  % Projection angle
\newcommand{\zzzR}{z_{\text R}}                         % Reconstruction position z_R

\newcommand{\CD}{180$^\circ$CD}
\newcommand{\CI}{180$^\circ$CI}
\newcommand{\MCD}{180$^\circ$MCD}
\newcommand{\MCI}{180$^\circ$MCI}
\newcommand{\MFI}{180$^\circ$MFI}
\newcommand{\MLI}{180$^\circ$MLI}

%\newcommand{\bpm}{\mbox{bpm}}                  % Beats per minute 
\newcommand{\bpm}{\mbox{min$^{-1}$}}            % Beats per minute
\newcommand{\fH}{f_{\text H}}                   % Heart rate

